A Case for Time Slotted Channel Hopping for ICN in the IoT

Recent proposals to simplify the operation of the IoT include the use of Information Centric Networking (ICN) paradigms. While this is promising, several challenges remain. In this paper, our core contributions (a) leverage ICN communication patterns to dynamically optimize the use of TSCH (Time Slotted Channel Hopping), a wireless link layer technology increasingly popular in the IoT, and (b) make IoT-style routing adaptive to names, resources, and traffic patterns throughout the network--both without cross-layering. Through a series of experiments on the FIT IoT-LAB interconnecting typical IoT hardware, we find that our approach is fully robust against wireless interference, and almost halves the energy consumed for transmission when compared to CSMA. Most importantly, our adaptive scheduling prevents the time-slotted MAC layer from sacrificing throughput and delay.

==> text/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
%Deploying ICN in the context of the Internet of Things is an enticing perspective.
Prior work has shown the potential and demonstrated the feasibility of ICN in the IoT, running directly on the MAC layer.
However, to fulfill this potential, the ICN network layer employed in this context needs to remain (i) lean and mean in terms of memory requirements and complexity, and (ii) allow advanced energy efficiency. 
In this view, combining ICN with a wireless MAC layer based on Time Slotted Channel Hopping (TSCH) is an enticing perspective.
The advantage of such a combination is two-fold.
On one hand, the reliability of TSCH avoids the need for complex error recovery mechanisms at the ICN layer.
On the other hand, TSCH combined with appropriate dynamic scheduling allows to be more energy efficient, while not incurring more delays, compared to typical contention-based MAC layers.
In this paper, we have thus designed mechanisms adjusting jointly, and on-the-fly, both TSCH time slot reservations and ICN Interest/Chunk multi-hop routing.
We have shown the efficiency of these mechanisms through experiments on state-of-the-art IoT hardware.
Compared to ICN on common contention-based MAC layers, we observed that our approaches (i) offer similar delay and throughput performance, but (ii) are more reliable and more predictable, and (iii) can reduce energy consumption by almost 50\%.

